What's Really Different with AI? -- A Behavior-based Perspective on System Safety for Automated Driving Systems

Assuring safety for ``AI-based'' systems is one of the current challenges in safety engineering. For automated driving systems, in particular, further assurance challenges result from the open context that the systems need to operate in after deployment. The current standardization and regulation landscape for ``AI-based'' systems is becoming ever more complex, as standards and regulations are being released at high frequencies. This position paper seeks to provide guidance for making qualified arguments which standards should meaningfully be applied to (``AI-based'') automated driving systems. Furthermore, we argue for clearly differentiating sources of risk between AI-specific and general uncertainties related to the open context. In our view, a clear conceptual separation can help to exploit commonalities that can close the gap between system-level and AI-specific safety analyses, while ensuring the required rigor for engineering safe ``AI-based'' systems.

==> fig/tikz/shapes.tex <==
%
% declare a new shape for the service interface
\makeatletter

\pgfdeclareshape{openinterface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
}
\pgfdeclareshape{interface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{.95\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
  \foregroundpath{
	 \centerpoint
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
    \pgfutil@tempdimb=\radius%      \pgfutil@tempdima = radius
	 \advance\pgfutil@tempdima by-.25\pgfutil@tempdima%
	 \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+.25\pgfutil@tempdimb}{0pt}}}{\pgfutil@tempdima}
	 \pgfusepath{fill}
  }
}
% UML component
\pgfdeclareshape{umlcomponent}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \backgroundpath{
	  \newdimen\pgf@xd\newdimen\pgf@yd
	  \newdimen\pgf@xe\newdimen\pgf@ye
	  \newdimen\pgf@xf\newdimen\pgf@yf
		% store lower right in xa/ya and upper right in xb/yb
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		% compute west point as well as vertical distance and height of decoration
		\pgf@xc=\pgf@xa \pgf@yc=.5\pgf@yb \advance\pgf@yc by .5\pgf@ya
		\pgf@yd=.3\pgf@yb
		\pgf@ye=.2\pgf@yb
%		% compute position of second decoration in xe/ye and xf/yf
%		\pgf@xe=\pgf@xa \pgf@ye=.1\pgf@y
%		\pgf@xf=\pgf@xa \pgf@yf=.2\pgf@ya
		% draw main shape
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathclose
		% draw internal lines
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
  }
}

% arrows
\pgfarrowsdeclare{srvarrow}{srvarrow}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.4\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.5\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{white}
  \pgfusepathqfill
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.8\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke
  \pgftransformshift{\pgfqpoint{-0.5\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.55\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill
}

\pgfarrowsdeclare{srvrequired}{srvrequired}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{1.3\pgfutil@tempdima}{0.95\pgfutil@tempdima}}}%
  \pgfpatharc{80}{280}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke 
}

\pgfarrowsdeclare{srvprovided}{srvprovided}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.4\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill 
}


\pgfdeclareshape{vehicle}
{
	 \savedanchor{\center}{
		\pgfpointorigin
	}
	\savedanchor{\cog}{
		\pgfpointadd{\pgfpointorigin}{\pgfpoint{-0.5cm}{0cm}}
	}
	\savedanchor{\origin}{
		\pgfpointadd{\pgfpointorigin}{\pgfpoint{-0.8cm}{0cm}}
	}
	\savedanchor{\front}{
		\pgfpointadd{\pgfpointorigin}{\pgfpoint{1.5cm}{0cm}}
	}
	\savedanchor{\rear}{
		\pgfpointadd{\pgfpointorigin}{\pgfpoint{-1.5cm}{0cm}}
	}
	\savedanchor{\upperleft}{
		\pgfpointadd{\pgfpointorigin}{\pgfpoint{-0.5cm}{0.5cm}}
	}
	\savedanchor{\lowerleft}{
		\pgfpointadd{\pgfpointorigin}{\pgfpoint{-0.5cm}{-0.5cm}}
	}
	\anchor{center}{\center}
	\anchor{cog}{\cog}
	\anchor{origin}{\origin}
	\anchor{front}{\front}
	\anchor{rear}{\rear}
	\anchor{west}{\left}
	\anchor{east}{\right}
	\backgroundpath{
    	\expandafter\let\expandafter\pgfsavedstrokecolor\csname\string\color@pgfstrokecolor\endcsname
		\pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
		\pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
		\pgftransformscale{8}
		\pgfpathmoveto{\pgfpointadd{\pgfpointorigin}{\pgfpoint{0.055cm}{-2.4}}}
		\pgfpathsvg{m 0,0 c 0.0308,0.13266 0.0758,0.27807 0.1092,0.37722 -0.007,0.003 -0.4436,-0.002 -0.97048,-0.0114 -0.87783,-0.0147 -1.03106,-0.0153 -1.82986,-0.004 -0.71279,0.01 -0.91136,0.01 -1.08934,10e-4 -0.39667,-0.0206 -0.77743,-0.003 -1.17616,0.0532 -0.0998,0.0142 -0.24948,0.0318 -0.33228,0.0398 -0.38256,0.0395 -0.75861,0.0824 -1.08417,0.1928 -0.12972,0.0803 -0.22624,0.1779 -0.27853,0.28112 -0.0492,0.0971 -0.15119,0.51145 -0.19379,0.78755 -0.0836,0.46772 -0.0505,0.99968 -5.2e-4,1.40567 0.0426,0.2761 0.14459,0.69045 0.19379,0.78755 0.0523,0.10322 0.14881,0.20082 0.27853,0.28112 0.32556,0.12455 0.7655,0.16241 1.08418,0.19271 0.0828,0.008 0.23248,0.0256 0.33228,0.0398 0.39873,0.0562 0.77948,0.0738 1.17615,0.0532 0.17798,-0.009 0.37655,-0.009 1.08934,0.001 0.7988,0.0112 0.95203,0.0106 1.82986,-0.004 0.52688,-0.009 0.96349,-0.0144 0.97049,-0.0114 -0.0372,0.12893 -0.079,0.26258 -0.1092,0.37721 0.0859,0.003 0.16072,0.002 0.20708,-0.006 0.10563,-0.1056 0.19121,-0.24562 0.2327,-0.38147 0.2485,-0.009 0.50354,-0.007 0.74672,-0.003 0.31623,0.0178 0.67684,0.007 1.05162,-0.031 0.31915,-0.0323 0.67421,-0.18303 0.94258,-0.40049 0.21095,-0.19094 0.3535,-0.37017 0.4987,-0.58703 0.0955,-0.68869 0.10307,-1.43594 10e-4,-2.02314 -0.13761,-0.22291 -0.32681,-0.41931 -0.4987,-0.58703 -0.26837,-0.21746 -0.62343,-0.36819 -0.94258,-0.40049 -0.37478,-0.038 -0.73538,-0.0488 -1.05161,-0.031 -0.27247,0.01 -0.47316,0.003 -0.74673,-0.003 -0.068,-0.20326 -0.17394,-0.32302 -0.21807,-0.35758 -0.0874,-0.0486 -0.11683,-0.0386 -0.2222,-0.0294 z}
	}
  \beforebackgroundpath{
	\pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
	\pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
	\pgfutil@definecolor{windowblue}{RGB}{168,196,196}
	\pgfpathmoveto{\pgfpointadd{\pgfpointorigin}{\pgfpoint{0.055cm}{-2.4}}}
	\pgfpathsvg{m -2.28723, 0.55668 c -0.32841,5e-5 -1.43918,0.0302 -1.48725,0.0403 -0.0232,0.005 -0.0231,0.006 0.0103,0.21187 l 0.0186,0.11473 0.15968,0.003 c 0.2659,0.005 1.31692,-0.0245 1.32912,-0.0367 0.0163,-0.0162 0.12751,-0.3088 0.12247,-0.32195 -0.003,-0.009 -0.0383,-0.0115 -0.15296,-0.0114 z m 0.6227,0.006 c -0.0219,0.0125 -0.26071,0.31771 -0.25528,0.32246 0.66703,0.003 1.41404,-0.0423 2.01745,-0.1746 0.0939,-0.022 0.10042,-0.0251 0.11731,-0.0537 0.0311,-0.0526 0.0299,-0.0533 -0.0992,-0.0594 -0.5927,-0.0184 -1.18929,-0.0423 -1.78028,-0.0348 z m -2.40708,0.0481 c -0.10328,-0.009 -1.36469,0.0745 -1.44695,0.0966 -0.0422,0.0113 -0.0811,0.0491 -0.0811,0.0718 0,0.01 0.012,0.039 0.0264,0.0641 v 5.2e-4 c 0.034,0.0594 0.0664,0.0743 0.18087,0.0847 0.0492,0.004 0.38906,0.008 0.7555,0.008 0.52523,2.3e-4 0.66715,-0.002 0.67025,-0.0109 0.002,-0.006 -0.0127,-0.079 -0.0336,-0.16174 l -0.0382,-0.15038 z m -2.64687,2.28254 c 0.0361,0.36599 0.11901,0.71377 0.21601,0.90641 0.0443,0.088 0.10539,0.17052 0.14469,0.19482 l 0.0315,0.0191 0.15555,-0.0987 c 0.0854,-0.0543 0.15554,-0.10194 0.15554,-0.10594 0,-0.004 -0.0144,-0.016 -0.032,-0.0269 -0.0664,-0.041 -0.14428,-0.17356 -0.19688,-0.33538 -0.0873,-0.26877 -0.1308,-0.64875 -0.13074,-1.02474 -7e-5,-0.376 0.0434,-0.75598 0.13074,-1.02475 0.0526,-0.16182 0.13051,-0.29436 0.19688,-0.33538 0.0176,-0.0109 0.032,-0.0229 0.032,-0.0269 0,-0.004 -0.0701,-0.0516 -0.15554,-0.10594 l -0.15555,-0.0987 -0.0315,0.0191 c -0.0393,0.0243 -0.1004,0.10685 -0.14469,0.19482 -0.097,0.19264 -0.17986,0.54042 -0.21601,0.90641 -0.0176,0.17802 -0.0194,0.2417 -0.0181,0.47129 -10e-4,0.22958 4.9e-4,0.29326 0.0181,0.47128 z m 6.24819,0.005 c -0.0174,0.28352 -0.0477,0.58871 -0.0796,0.79891 h -0.001 c -0.0235,0.15794 -0.0261,0.18934 -0.0155,0.19534 0.004,0.002 0.0341,0.007 0.0682,0.01 0.13705,0.0137 0.58706,0.0779 0.9338,0.13332 0.202,0.0323 0.39156,0.0587 0.42116,0.0589 0.1653,0.001 0.3057,-0.16225 0.41031,-0.47853 0.1047,-0.31587 0.15499,-0.75432 0.15399,-1.19062 v -0.006 c 0.001,-0.4363 -0.0493,-0.87476 -0.15399,-1.19063 -0.10461,-0.31628 -0.24501,-0.47978 -0.41031,-0.47852 -0.0296,2.3e-4 -0.21917,0.0266 -0.42117,0.0589 -0.34674,0.0554 -0.79674,0.11964 -0.93379,0.13332 -0.0341,0.003 -0.0645,0.008 -0.0682,0.01 -0.0106,0.006 -0.008,0.0374 0.0155,0.19534 h 0.001 c 0.0319,0.2102 0.0622,0.5154 0.0796,0.79892 0.0129,0.32362 0.009,0.63395 0,0.95188 z m -4.16667,1.00975 c -0.36644,0 -0.7063,0.004 -0.7555,0.008 -0.11447,0.0104 -0.14687,0.0253 -0.18087,0.0847 v 5.3e-4 c -0.0144,0.0251 -0.0264,0.0541 -0.0264,0.0641 0,0.0227 0.0389,0.0605 0.0811,0.0718 0.0823,0.0221 1.34367,0.10564 1.44695,0.0966 l 0.0331,-0.003 0.0382,-0.15037 c 0.0209,-0.0827 0.0356,-0.15575 0.0336,-0.16175 -0.003,-0.009 -0.14502,-0.0111 -0.67025,-0.0109 z m 1.0511,0.01 -0.15968,0.003 -0.0186,0.11472 c -0.0334,0.20587 -0.0335,0.20688 -0.0103,0.21188 0.0481,0.0101 1.15883,0.0403 1.48724,0.0403 0.11466,1e-4 0.14997,-0.002 0.15297,-0.0114 0.005,-0.0131 -0.10618,-0.30575 -0.12248,-0.32195 -0.0122,-0.0122 -1.06322,-0.0417 -1.32912,-0.0367 z m 1.66605,0.0413 c 0.0964,0.14656 0.23338,0.30996 0.25528,0.32246 0.0201,0.0115 1.34512,-0.0143 1.78026,-0.0346 0.1291,-0.006 0.13032,-0.007 0.0992,-0.0594 -0.0169,-0.0286 -0.0234,-0.0317 -0.11731,-0.0537 -0.59115,-0.0993 -1.33329,-0.16979 -2.01743,-0.17476 z}
	\pgfsetcolor{windowblue}

	\begingroup
		\tikz@mode
		\iftikz@mode@draw
			\expandafter\pgf@setstrokecolor\pgfsavedstrokecolor
			\pgfusepath{stroke, fill}
		\else
			\pgfusepath{fill}
		\fi
	\endgroup
}
}
\newdimen\ya
\newdimen\xa
\newdimen\lastangle
\newdimen\pgfdecorationlanewidth
\makeatletter
%\pgfmathparse{10*\pgflinewidth}
\pgfdecorationlanewidth10\pgflinewidth
%
\newif\ifpgfdecoratehascenterline
\pgfkeys{%
	/pgf/decoration/.cd,
	lane width/.code={\pgfmathsetlength\pgfdecorationlanewidth{#1}},
	outer modulation/.default=1,
	outer modulation/.store in=\pgfdecorationlanemodulation,
	outer modulation,
	draw centerline/.is if=pgfdecoratehascenterline,
	draw centerline=true,
}
\pgfdeclaredecoration{road}{initial}
{
	\state{initial}[%
	width=\pgfdecorationsegmentlength, %
	next state=curve, %
	persistent postcomputation={
		%store the next control point
		\pgfmathsetlength{\lastangle}{\pgfdecoratedangle}%
	}
	]{
		\pgfpathmoveto{\pgfpointorigin}
		%calculate the next control point
		\pgfcoordinate{@1}{\pgfpoint{0pt}{0pt}}
		\pgfcoordinate{@2}{\pgfpoint{.3\pgfdecorationsegmentlength}{0pt}}
		\pgfcoordinate{@3}{\pgfpoint{0pt}{\pgfdecorationlanewidth}}
		\pgfcoordinate{@4}{\pgfpoint{.4\pgfdecorationsegmentlength}{\pgfdecorationlanewidth}}
		\pgfcoordinate{@5}{\pgfpoint{0pt}{-\pgfdecorationlanewidth}}
		\pgfcoordinate{@6}{\pgfpoint{.4\pgfdecorationsegmentlength}{-\pgfdecorationlanewidth}}
		\pgf@process{\pgfpointtransformed{\pgfpoint{0}{0}}}
		%\pgfmathsetmacro{\lastangle}{\pgfdecoratedangletonextinputsegment}
	}
	%
	\state{curve}[%
	width=\pgfdecorationsegmentlength,
	next state=curve,
	switch if less than=\pgfdecorationsegmentlength to final,
	persistent postcomputation={
		%store the next control point
		\pgfmathsetlength{\lastangle}{\pgfdecoratedangle}%
	}
	]{	
		%
		%
		\edef\curlinewidth{\the\pgflinewidth}
		\pgfmathsetlengthmacro\pgf@decoration@contour@shorten{%
			\pgfdecorationlanewidth*sin((\pgfdecoratedangle-\lastangle))}
		\begin{pgfscope}
			\pgfpathmoveto{\pgfpoint{0}{0}}
			\pgfsetlinewidth{2.4\pgfdecorationlanewidth}
			\pgfpathlineto{\pgfpointanchor{@1}{center}}
			\pgfsetstrokecolor{lightgray}
			\pgfpathmoveto{\pgfpoint{\pgf@decoration@contour@shorten}{1.2*\pgfdecorationlanewidth}}
			\pgfpathlineto{\pgfpoint{0}{1.2\pgfdecorationlanewidth}}
			\pgfpathmoveto{\pgfpoint{\pgf@decoration@contour@shorten}{1.2*\pgfdecorationlanewidth}}
			\pgfusepath{stroke}
		\end{pgfscope}
		%
		\pgfpathmoveto{\pgfpoint{0}{0}}
		%
		\pgfpathmoveto{\pgfpoint{0.2}{0}}
		%
		\begin{pgfscope}
			\pgfsetlinewidth{\curlinewidth}
			\pgfsetstrokecolor{white}
			%
			\ifpgfdecoratehascenterline
			\pgfpathcurvebetweentime{0.5}{1}{%
				\pgfpoint{0.0}{0}
			}%
			{%
				\pgfpoint{-.3\pgfdecorationsegmentlength}{0pt}%
			}%
			{%
				\pgfpointanchor{@2}{center}%
			}%
			{%
				\pgfpointanchor{@1}{center}%
			}%
			\fi
			%
			\newdimen\dummy
			\dummy = \pgfdecorationlanemodulation pt
			\ifdim\dummy>0.0pt
			\pgfpathmoveto{\pgfpoint{0}{\pgfdecorationlanewidth}}
			\pgfpathcurvebetweentime{0}{\pgfdecorationlanemodulation}{%
				\pgfpoint{0}{\pgfdecorationlanewidth}
			}%
			{%
				\pgfpoint{-.5\pgfdecorationsegmentlength}{\pgfdecorationlanewidth}%
			}%
			{%
				\pgfpointanchor{@4}{center}%
			}%
			{%
				\pgfpointanchor{@3}{center}%
			}%
			\pgfpathmoveto{\pgfpoint{0}{-\pgfdecorationlanewidth}}
			\pgfpathcurvebetweentime{0}{\pgfdecorationlanemodulation}{%
				\pgfpoint{0}{-\pgfdecorationlanewidth}
			}%
			{%
				\pgfpoint{-.5\pgfdecorationsegmentlength}{-\pgfdecorationlanewidth}%
			}%
			{%
				\pgfpointanchor{@6}{center}%
			}%
			{%
				\pgfpointanchor{@5}{center}%
			}%	
			%
			\fi
			\pgfusepath{stroke}
		\end{pgfscope}
		%
		\pgfcoordinate{@1}{\pgfpoint{-0.5pt}{0pt}}
		\pgfcoordinate{@2}{\pgfpoint{.3\pgfdecorationsegmentlength}{0pt}}
		\pgfcoordinate{@3}{\pgfpoint{-0.7pt}{\pgfdecorationlanewidth}}
		\pgfcoordinate{@4}{\pgfpoint{.4\pgfdecorationsegmentlength}{\pgfdecorationlanewidth}}
		\pgfcoordinate{@5}{\pgfpoint{-0.7pt}{-\pgfdecorationlanewidth}}
		\pgfcoordinate{@6}{\pgfpoint{.4\pgfdecorationsegmentlength}{-\pgfdecorationlanewidth}}
	}
	\state{final}
	{%
		\edef\curlinewidth{\the\pgflinewidth}
		\begin{pgfscope}
			\pgfpathmoveto{\pgfpoint{\pgfdecoratedremainingdistance}{0}}
			\pgfsetlinewidth{2.4\pgfdecorationlanewidth}
			\pgfpathlineto{\pgfpointanchor{@1}{center}}
			\pgfsetstrokecolor{lightgray}
			\pgfusepath{stroke}
		\end{pgfscope}
		%
		\pgfpathmoveto{\pgfpoint{0}{0}}
		%
		\pgfpathmoveto{\pgfpoint{0.2}{0}}
		%
		\begin{pgfscope}
			\pgfsetlinewidth{\curlinewidth}
			\pgfsetstrokecolor{white}
			\ifpgfdecoratehascenterline
			\pgfpathcurvebetweentime{0.5}{1}{%
				\pgfpoint{0.0}{0}
			}%
			{%
				\pgfpoint{-.3\pgfdecorationsegmentlength}{0pt}%
			}%
			{%
				\pgfpointanchor{@2}{center}%
			}%
			{%
				\pgfpointanchor{@1}{center}%
			}%
			\fi
			%
			\newdimen\dummy
			\dummy = \pgfdecorationlanemodulation pt
			\ifdim\dummy>0.0pt
			\pgfpathmoveto{\pgfpoint{\pgfdecoratedremainingdistance}{\pgfdecorationlanewidth}}
			\pgfpathcurvebetweentime{0}{\pgfdecorationlanemodulation}{%
				\pgfpoint{\pgfdecoratedremainingdistance}{\pgfdecorationlanewidth}
			}%
			{%
				\pgfpoint{-.5\pgfdecorationsegmentlength}{\pgfdecorationlanewidth}%
			}%
			{%
				\pgfpointanchor{@4}{center}%
			}%
			{%
				\pgfpointanchor{@3}{center}%
			}%
			%	
			\pgfpathmoveto{\pgfpoint{\pgfdecoratedremainingdistance}{-\pgfdecorationlanewidth}}
			\pgfpathcurvebetweentime{0}{\pgfdecorationlanemodulation}{%
				\pgfpoint{\pgfdecoratedremainingdistance}{-\pgfdecorationlanewidth}
			}%
			{%
				\pgfpoint{-.5\pgfdecorationsegmentlength}{-\pgfdecorationlanewidth}%
			}%
			{%
				\pgfpointanchor{@6}{center}%
			}%
			{%
				\pgfpointanchor{@5}{center}%
			}%	
			%
			\fi
			\ifpgfdecoratehascenterline
			\ifdim\pgfdecoratedinputsegmentremainingdistance<\pgfdecorationsegmentlength*0.55
			\pgfmoveto{\pgfpoint{\pgfdecoratedinputsegmentremainingdistance}{0}}
			\pgflineto{\pgfpoint{0}{0}}
			\fi
			\fi
			\pgfusepath{stroke}
		\end{pgfscope}	
	}
}

\pgfkeys{/pgf/.cd,
	parallelepiped offset x/.initial=2mm,
	parallelepiped offset y/.initial=2mm
}
\pgfdeclareshape{parallelepiped}
{
	\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
	\inheritanchorborder[from=rectangle]
	\inheritanchor[from=rectangle]{north}
	\inheritanchor[from=rectangle]{north west}
	\inheritanchor[from=rectangle]{north east}
	\inheritanchor[from=rectangle]{center}
	\inheritanchor[from=rectangle]{west}
	\inheritanchor[from=rectangle]{east}
	\inheritanchor[from=rectangle]{mid}
	\inheritanchor[from=rectangle]{mid west}
	\inheritanchor[from=rectangle]{mid east}
	\inheritanchor[from=rectangle]{base}
	\inheritanchor[from=rectangle]{base west}
	\inheritanchor[from=rectangle]{base east}
	\inheritanchor[from=rectangle]{south}
	\inheritanchor[from=rectangle]{south west}
	\inheritanchor[from=rectangle]{south east}
	\backgroundpath{
		% store lower right in xa/ya and upper right in xb/yb
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/parallelepiped offset x}}
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/parallelepiped offset y}}
		\def\ppd@offset{\pgfpoint{\pgfutil@tempdima}{\pgfutil@tempdimb}}
		\pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathclose
		\pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@ya}}{\ppd@offset}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xa}{\pgf@yb}}{\ppd@offset}}
		\pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
	}
}

\makeatother
